Permutation-Invariant Tabular Data Synthesis

Tabular data synthesis is an emerging approach to circumvent strict regulations on data privacy while discovering knowledge through big data. Although state-of-the-art AI-based tabular data synthesizers, e.g., table-GAN, CTGAN, TVAE, and CTAB-GAN, are effective at generating synthetic tabular data, their training is sensitive to column permutations of input data. In this paper, we first conduct an extensive empirical study to disclose such a property of permutation invariance and an in-depth analysis of the existing synthesizers. We show that changing the input column order worsens the statistical difference between real and synthetic data by up to 38.67% due to the encoding of tabular data and the network architectures. To fully unleash the potential of big synthetic tabular data, we propose two solutions: (i) AE-GAN, a synthesizer that uses an autoencoder network to represent the tabular data and GAN networks to synthesize the latent representation, and (ii) a feature sorting algorithm to find the suitable column order of input data for CNN-based synthesizers. We evaluate the proposed solutions on five datasets in terms of the sensitivity to the column permutation, the quality of synthetic data, and the utility in downstream analyses. Our results show that we enhance the property of permutation-invariance when training synthesizers and further improve the quality and utility of synthetic data, up to 22%, compared to the existing synthesizers.

==> chapters/feature_sorting.tex <==
\label{feature_sorting_algorithm}
%\lc{shorten this by half, especially the algorithm environment}
Although features in tabular data are often heterogeneous, some are highly correlated, such as age and experience, or height and weight. However, as discussed in Section~\ref{cnn_not_a_natural_fit}, CNN-based tabular data synthesizers often fail to capture these correlations due to their focus on local relations. A simple solution for this problem is to put highly-correlated features together, such that a convolution kernel can capture them simultaneously. 

The location of features also matters in CNNs. In a convolution process, the features on the border of the input matrix are convoluted fewer times than the features within the border, leading to potential loss of information about features on the border. This is called \textit{boundary effects} in image processing~\cite{castleman1996digital, strang1996wavelets}. Previous studies have shown that boundary effects result in statistical biases in finite-sampled data~\cite{kayhan2020translation, griffith1983boundary, griffith1983evaluation}.
%, and various methods have been proposed to reduce its impact~\cite{innamorati2020learning, cheng2018cube, schubert2019circular}. Therefore, 
To better capture the correlation between features, one must also carefully choose the location of high-correlated features. 

Our solution is to group highly-correlated features together in the middle of the table. This brings two advantages: (1) A convolution kernel can capture highly-correlated features simultaneously so that their correlation is better preserved; and (2) highly-correlated features will be located at the center of the input matrix and be less prone to the boundary effects.% in CNNs. 

Figure~\ref{fig:put_high_corr_cols_in_mid} illustrates the base of our idea. Take one table row as an example. We reshape it into a square matrix to feed it to a CNN. Before reshaping, two pairs of highly correlated features, $\{F1, F2\}$ and $\{F15, F16\}$, are at the leftmost and rightmost locations. As a result, they are on the border of the input matrix after reshaping. Due to the boundary effects in CNNs, the correlations between $F1$ and $F2$, and $F15$ and $F16$ are probably lost after several aggregations, activation, and pooling operations. However, by putting $\{F1, F2\}$ and $\{F15, F16\}$ in the middle of the row they end up at the center of the input matrix. This ensures that they are close by and less susceptible to boundary effects.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{images/high_corr_in_middle.drawio.pdf}
    \caption{\textbf{Top: }The highly correlated features, $F1, F2, F15$ and $F16$ are on the border of the input matrix, suffering from the boundary effects of CNNs. \textbf{Bottom: }After feature sorting, $F1, F2, F15$ and $F16$ are at the center of the input matrix.}
    \label{fig:put_high_corr_cols_in_mid}
\end{figure}

Although this idea seems straightforward, one complication arises due to the encoding of features. Variational Gaussian Mixture~\cite{ctgan&tvae} and One-hot encoding require multiple columns to represent one feature. Consequently, each feature may occupy a different number of columns. To put highly correlated features in the middle after encoding, we must consider the length of each encoded feature.

We developed a feature sorting algorithm that groups  highly-correlated features and puts them in the middle, see Algorithm~\ref{alg:feature_sort}. %In this algorithm, 
We first pick the most correlated feature pairs and then add other features to their left or right side. We have two counters, $c_{left}$ and $c_{right}$, for columns taken by features added to the left and the right side. Before adding a feature, we compare $c_{left}$ and $c_{right}$, and then add it to the side with fewer columns. Thereby we ensure that the highly correlated features stay in the middle even after encoding.

\begin{algorithm}[h]
\caption{Feature Sorting Algorithm} %: Put highly-correlated features in the middle}
\label{alg:feature_sort}
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \Require Original Table $T_o = \{F_0, F_1, ..., F_n\}$
 \Ensure  Sorted Table $T_{sorted}$
   \State $T_{sorted} \gets \{\}$
   \State $c_{left}, c_{right} \gets 0$ \Comment{No. columns added to the left / right of $T_{sorted}$}
   \State $corr \gets [~]$ \Comment{Pair-wise correlation / association}
   \For {all possible pairs of features in $T_o$}
   \State Calculate the absolute value of their correlation / association and save it in $corr$
   \EndFor
   \While {$length(T_{sorted}) \neq length(T_{o})$ }
   \State Find the largest value $v$ in $corr$
   \State Find the corresponding pair of features $\{F_x, F_y\}$
   \State $F_{new} \gets \{F_x, F_y\} - \{F_x, F_y\} \cap T_{sorted}$ \Comment{Feature(s) not yet in $T_{sorted}$}
   \State $c \gets$ No. columns occupied by $F_{new}$ after encoding
    \If {$T_{sorted}$ is empty}
    \State $T_{sorted} \gets \{F_x, F_y\}$ \Comment{Add the first pair}
    \Else
    \If {$c_{right} < c_{left}$}
    \State $T_{sorted} \gets T_{sorted} + F_{new}$ \Comment{Add the new feature(s) to the right}
    \State $c_{right} \gets c_{right} + c$
    \Else
    % \State Add $F_x$ and $F_y$ to the left of $T_{sorted}$
    \State $T_{sorted} \gets  F_{new} + T_{sorted}$ \Comment{Add the new feature(s) to the left}
    \State $c_{left} \gets c_{left} + c$
    \EndIf
    \EndIf
    \State Remove $v$ from $corr$
   \EndWhile
 \State \Return $T_{sorted}$ 
 \end{algorithmic} 
\end{algorithm}
